Using Psychological Characteristics of Situations for Social Situation Comprehension in Support Agents

Support agents that help users in their daily lives need to take into account not only the user's characteristics, but also the social situation of the user. Existing work on including social context uses some type of situation cue as an input to information processing techniques in order to assess the expected behavior of the user. However, research shows that it is important to also determine the meaning of a situation, a step which we refer to as social situation comprehension. We propose using psychological characteristics of situations, which have been proposed in social science for ascribing meaning to situations, as the basis for social situation comprehension. Using data from user studies, we evaluate this proposal from two perspectives. First, from a technical perspective, we show that psychological characteristics of situations can be used as input to predict the priority of social situations, and that psychological characteristics of situations can be predicted from the features of a social situation. Second, we investigate the role of the comprehension step in human-machine meaning making. We show that psychological characteristics can be successfully used as a basis for explanations given to users about the decisions of an agenda management personal assistant agent.

==> model_accuracy.tex <==
\newcolumntype{b}{X}
\newcolumntype{Y}{>{\hsize=.95\hsize}X}
\newcolumntype{s}{>{\centering\arraybackslash}Y}

\begin{table}[!h]
\caption{Mean Absolute Errors of the models in predicting the psychological characteristics of situations. Psychological characteristics marked with * represent statistically different results between the two models (Wilcoxon Rank sum test, $p<0.05$). }
\centering
\begin{tabularx}{0.65\textwidth}{bss}
\hline
Psychological \\ Characteristic                     & \begin{tabular}[c]{@{}c@{}}Random Forest\end{tabular} & \begin{tabular}[c]{@{}c@{}}Predict Mean\end{tabular} \\ \hline
Duty*         & 1.34                                                           & 1.55                                                          \\
Intellect* & 1.17                                                          & 1.3                                                           \\
Adversity              & 1.29                                                           & 1.36                                                          \\
Mating*             & 0.85                                                           & 1.03                                                          \\
Positivity*             & 1.14                                                           & 1.26                                                          \\
Negativity*             & 1.25                                                           & 1.37                                                          \\
Deception             & 1.04                                                           & 1.09                                                          \\
Sociality*                   & 1.02                                                           & 1.13                                                          \\ \hline
\end{tabularx}
\label{model_accuracies}
\end{table}

==> priority_accuracy.tex <==
\newcolumntype{b}{X}
\newcolumntype{Y}{>{\hsize=.32\hsize}X}
\newcolumntype{s}{>{\centering\arraybackslash}Y}

\begin{table}[!h]
\caption{Mean Absolute Errors of the models in predicting the priority of social situations when using different inputs. Results marked with * are significantly different from the others (Wilcoxon Rank sum test, $p<0.05$).}
\centering
\begin{tabularx}{0.95\textwidth}{bs}
\hline
Model input                     & \begin{tabular}[c]{@{}c@{}}Mean Absolute Error \\ in Priority Prediction\end{tabular} \\ \hline
Social situation features \citep{kola2020predicting}         & 1.35                                                                                             \\
True psychological characteristics of situations  & 0.98*                                                                                                                     \\
Predicted psychological characteristics of situations                                                             & 1.37                              
                                                          \\ \hline
\end{tabularx}
\label{priority_accuracies}
\end{table}
